Learning Neural Networks with Two Nonlinear Layers in Polynomial Time

We give a polynomial-time algorithm for learning neural networks with one layer of sigmoids feeding into any Lipschitz, monotone activation function (e.g., sigmoid or ReLU). We make no assumptions on the structure of the network, and the algorithm succeeds with respect to {\em any} distribution on the unit ball in $n$ dimensions (hidden weight vectors also have unit norm). This is the first assumption-free, provably efficient algorithm for learning neural networks with two nonlinear layers. Our algorithm-- {\em Alphatron}-- is a simple, iterative update rule that combines isotonic regression with kernel methods. It outputs a hypothesis that yields efficient oracle access to interpretable features. It also suggests a new approach to Boolean learning problems via real-valued conditional-mean functions, sidestepping traditional hardness results from computational learning theory. Along these lines, we subsume and improve many longstanding results for PAC learning Boolean functions to the more general, real-valued setting of {\em probabilistic concepts}, a model that (unlike PAC learning) requires non-i.i.d. noise-tolerance.

==> files/app.tex <==
The general framework of the previous section can be used to give new learning results for well studied problems. In this section we give polynomial time learnability results for neural networks with two sigmoidal layers in the p-concept model.


==> files/conclusion.tex <==
We have given the first assumption-free, polynomial-time algorithm for
learning a class of non-linear neural networks with more than one
hidden layer.  We only require that the conditional mean function is
computed by such a network, and therefore our results also capture Boolean
learning problems.  In contrast, PAC learning corresponding Boolean
{\em function classes} seems intractable.

Understanding the broadest class of conditional mean functions that
admit efficient learning algorithms is a natural open problem.  For
example, can we learn two hidden layers with multiple hidden units in the
second layer?  

We remark that while our algorithms are noise-tolerant in the
sense that we make assumptions only on the conditional mean function,
it is unlikely that our results can be extended to the fully
non-realizable (agnostic) setting, as there are hardness results for
agnostically learning even a single ReLU in fully-polynomial time
\cite{goel2016reliably}.

Finally, it is easy to see that depth-$3$ neural networks with one
hidden layer of ReLUs feeding into a sigmoid can approximate (with
negligible error), polynomial-size DNF formulas.  Thus, it is unlikely
we can obtain polynomial-time algorithms for such architectures
\cite{DanielyS16}.

==> files/pac.tex <==
Consider $t$-halfspaces $\{h_1, \ldots, h_t\}$. An intersection of these $t$-halfspaces is given by $f_{\mathsf{AND}}(\textbf{x}) = \wedge_{i=1}^t h_{i}(\textbf{x})$. A majority of $t$-halfspaces is given by $f_{\mathsf{maj}}(\textbf{x}) =\mathsf{sign}\left(\sum_{i=1}^t h_i(\textbf{x}) - t/2 \right)$.

The following lemmas show that there exists kernels that separate intersection/majority of halfspaces.
\begin{lemma} \label{lem:interpac}
Intersection of $t$-halfspaces on $\S^{n-1}$ is $B$-separated by a kernel $\mathcal{K}$ such that $\forall \textbf{x} \in \mathcal{H}, \mathcal{K}(\textbf{x}, \textbf{x}) \leq 1$ with $B = t^{O(\sqrt{1/\rho})}$.
\end{lemma}
\begin{proof}
%The proof follows from showing that for a particular $u$, the distribution of data is identical to the given data and subsequently applying Theorem \ref{thm:fhs} to learn this class. Finally, we will show how to go from squared loss to $0-1$ loss.
Consider $P_{\mathsf{AND}}$ given by Lemma \ref{lem:inter} for given $\rho$. We know that $\forall \textbf{x} \in \S^{n-1}$, $P_{\mathsf{AND}}(\textbf{x}) \geq 1/2$ if $f_{\mathsf{AND}}(\textbf{x}) = 1$ and  $P_{\mathsf{AND}}(\textbf{x}) \leq -1/2$ if $f_{\mathsf{AND}}(\textbf{x}) = 0$. We know that each coefficient of $T_r(a)$ is bounded by $2^r$. It is easy to see that each coefficient of $T_r(1-a)$ is bounded by $2^{O(r)}$. Using Lemma \ref{lem:rbound}, the sum of squares of the coefficients of $p(a)$ are bounded by $2^{O(r{\lceil \log 2t \rceil})} = t^{O(r)}$. Now using Lemma \ref{lem:Bbound}, we know that $p(\textbf{w}_\textbf{i} \cdot \textbf{x}) = \langle \textbf{v}_\textbf{i}, \psi_d(\textbf{x}) \rangle$ for the feature vector $\psi_d$ of the multinomial kernel with $d = r{\lceil \log 2t \rceil}$. such that $||\textbf{v}_\textbf{i}|| \leq t^{O(r)}$. Thus, $P_{\mathsf{AND}}(\textbf{x}) = \langle \textbf{v}, \psi_d(\textbf{x}) \rangle$ (adjusting the constant term corresponding to the 1 entry in the feature vector) such that $||\textbf{v}|| \leq t^{O(r)}$. We can assume that $||\psi(\textbf{x})|| \leq 1$ by scaling the weight vector appropriately as before. Thus, $f_{\mathsf{AND}}$ is $t^{O(r)}$-separated by kernel $\mathcal{MK}_d$.
\end{proof}

\begin{lemma} \label{lem:maj}
Majority of $t$-halfspaces on $\S^{n-1}$ is $B$-separated by a kernel $\mathcal{K}$ such that $\forall \textbf{x} \in \mathcal{H}, \mathcal{K}(\textbf{x}, \textbf{x}) \leq 1$ with $B = t^{O(1/\rho)}$.
\end{lemma}
\begin{proof}
%The proof follows from showing that for a particular $u$, the distribution of data is identical to the given data and subsequently applying Theorem \ref{thm:fhs} to learn this class. Finally, we will show how to go from squared loss to $0-1$ loss.

We use Lemma \ref{lem:approxsign} to show the existence of polynomial $p$ of degree $d = O\left( \frac{1}{\rho} \cdot \log t \right)$ such that for $a \in [−1, 1]$, $|p(a)| < 1 + 1/2t$ and for $a \in [−1, 1] \ [-\rho, \rho]$, $|p(a) − \mathsf{sign}(a)| < 1/2t$. Consider
\[
P_\mathsf{maj}(\textbf{x}) = \sum_{i=1}^t p(\textbf{w}_\textbf{i} \cdot \textbf{x}) - \frac{t}{2}
\]
Since for each $h_i$, $\rho \leq |\textbf{w}_\textbf{i} \cdot \textbf{x}| \leq 1$, we have $|p(\textbf{w}_\textbf{i} \cdot \textbf{x}) − \mathsf{sign}(\textbf{w}_\textbf{i} \cdot \textbf{x})| \leq 1/2t$. Thus if $f_{\mathsf{maj}}(\textbf{x}) = 1$ then $P_\mathsf{maj}(\textbf{x}) \geq \sum_{i=1}^t h_i(\textbf{x}) - t/2  - 1/2 \geq 1/2$. Similarly if $f_{\mathsf{maj}}(\textbf{x}) = 0$ then $P_\mathsf{maj}(\textbf{x}) \leq - 1/2$.

From Lemma \ref{lem:dbound} and \ref{lem:Bbound}, we have that for each $i$, $p(\textbf{w}_\textbf{i} \cdot \textbf{x}) = \langle \textbf{v}_\textbf{i}, \psi(\textbf{x}) \rangle$ such that $|| \textbf{v}_\textbf{i} || = t^{O(1/\rho)}$ where $\psi$ is the feature vector corresponding to the multinomial kernel of degree $d$. Thus, $P_\mathsf{maj}(\textbf{x}) = \langle \textbf{v}, \psi(\textbf{x}) \rangle$ (adjusting the constant term corresponding to the 1 entry in the feature vector) such that $||\textbf{v}|| = t^{O(1/\rho)}$. We can assume that $||\psi(\textbf{x})| \leq 1$ by scaling the weight vector appropriately as before. Thus, $f_{\mathsf{maj}}$ is $t^{O(1/\rho)}$-approximated by kernel $\mathcal{K}$.
\end{proof}

Applying Theorem \ref{thm:pac} to the above lemmas, we obtain the following results for PAC learning:
\begin{corollary}
There exists an algorithm that PAC learns any intersection of $t$-halfspaces with margin $\rho>0$ on $\S^{n-1}$ in time $t^{O(\sqrt{1/\rho})} \cdot poly(n, 1/\epsilon, \log(1/\delta))$.
\end{corollary}

This result improves the previous best bound by \cite{klivans2008learning} that had running time roughly $n \cdot \left(\frac{\log t}{\rho}\right)^{O\left(\sqrt{\frac{1}{\rho}} \log t\right)}$. For constant $\rho$, our algorithm is the first that has running time polynomial in the number of halfspaces.

\begin{corollary}
There exists an algorithm that PAC learns any majority of $t$-halfspaces with margin $\rho>0$ on $\S^{n-1}$ in time $t^{O(\sqrt{1/\rho})} \cdot poly(n, 1/\epsilon, \log(1/\delta))$.
\end{corollary}

==> files/prelims.tex <==
\subsection{Learning Models}
We consider two learning models in our paper, the standard Probably Approximately Correct (PAC) learning model and a relaxation of the standard model, the Probabilistic Concept (p-concept) learning model. For completeness, we define the two models and refer the reader to \cite{valiant1984theory,kearns1990efficient} for a detailed explanation.
\begin{definition}[PAC Learning \cite{valiant1984theory}] 
	We say that a concept class $\mathcal{C} \subseteq
        \{0,1\}^{\mathcal{X}}$ is Probably Approximately Correct (PAC)
        learnable, if there exists an algorithm $\mathcal{A}$ such
        that for every $c \in \mathcal{C}$,$\delta, \epsilon >
	0$ and $\mathcal{D}$ over $\mathcal{X}$, if $\mathcal{A}$ is given access
	to examples drawn from $\mathcal{D}$ and labeled according to $c$, $\mathcal{A}$ outputs a hypothesis $h : \mathcal{X}
	\rightarrow \{0,1\}$, such that with probability at least $1 - \delta$,
	%
	\begin{equation}
		%%
		  Pr_{\textbf{x} \sim \mathcal{D}} [h(\textbf{x}) \neq c(\textbf{x})] \leq \epsilon.
		%%
	\end{equation}
	%
	Furthermore, we say that $\mathcal{C}$ is \emph{efficiently PAC learnable to error
	$\epsilon$} if $\mathcal{A}$ can output an $h$ satisfying the
      above with running time and sample complexity polynomial in $n$, $1/\epsilon$, and
	$1/\delta$.
\end{definition}

\begin{definition}[p-concept Learning \cite{kearns1990efficient}] 
	We say that a concept class $\mathcal{C} \subseteq
        \mathcal{Y}^{\mathcal{X}}$ is Probabilistic Concept
        (p-concept) learnable, if there exists an algorithm
        $\mathcal{A}$ such that for every $\delta, \epsilon >
	0$, $c \in \mathcal{C}$ and
	distribution $\mathcal{D}$ over $\mathcal{X} \times
        \mathcal{Y}$ with $\E[y|\textbf{x}] = c(\textbf{x})$ we have
        that $\mathcal{A}$, given access
	to examples drawn from $\mathcal{D}$, outputs a hypothesis $h : \mathcal{X}
	\rightarrow \mathcal{Y}$, such that with probability at least $1 - \delta$,
	%
	\begin{equation}
		%%
		  \E_{(\textbf{x},y) \sim \mathcal{D}} [(h(\textbf{x}) - c(\textbf{x}))^2] \leq  \epsilon.
		%%
	\end{equation}
	%
	Furthermore, we say that $\mathcal{C}$ is \emph{efficiently p-concept learnable to error
	$\epsilon$} if $\mathcal{A}$ can output an $h$ satisfying the
      above with running time and sample complexity polynomial in $n$, $1/\epsilon$, and
	$1/\delta$.
\end{definition}
Here we focus on square loss for p-concept since an efficient algorithm for square-loss implies efficient algorithms of various other standard losses.

\subsection{Generalization Bounds}
The following standard generalization bound based on Rademacher complexity is useful for our analysis. For a background on Rademacher
complexity, we refer the readers to \cite{BM:2002}.

\begin{theorem}[\cite{BM:2002}] \label{generalizationbound}
	%%
	Let $\mathcal{D}$ be a distribution over $\mathcal{X} \times \mathcal{Y}$ and let $\mathcal{L} : \mathcal{Y}^\prime
	\times \mathcal{Y}$ (where $\mathcal{Y} \subseteq \mathcal{Y}^\prime \subseteq \mathbb{R}$) be a
	$b$-bounded loss function that is $L$-Lipschitz in its first argument.  Let
	$\mathcal{F} \subseteq (\mathcal{Y}^\prime)^\mathcal{X}$ and for any $f \in \mathcal{F}$, let $\mathcal{L}(f; \mathcal{D}) := \E_{(\textbf{x}, y)
	\sim \mathcal{D}}[\mathcal{L}(f(\textbf{x}), y)]$ and $\hat{\mathcal{L}}(f; S) := \frac{1}{m} \sum_{i = 1}^m
	\mathcal{L}(f(\textbf{x}_\textbf{i}), y_i)$, where $S = ((\textbf{x}_\textbf{1}, y_1), \ldots,  (\textbf{x}_\textbf{m}, y_m))  \sim
	\mathcal{D}^m$. Then for any $\delta > 0$, with probability at least $1 - \delta$
	(over the random sample draw for $S$), simultaneously for all $f \in
	\mathcal{F}$, the following is true:
	%%
	\[
		|\mathcal{L}(f; \mathcal{D}) - \hat{\mathcal{L}}(f; S)| \leq 4 \cdot L \cdot \mathcal{R}_\textbf{m}(\mathcal{F})
		+ 2\cdot b \cdot \sqrt{\frac{\log (1/\delta)}{2m}}
	\]
	where $\mathcal{R}_\textbf{m}(\mathcal{F})$ is the Rademacher complexity of the function class $\mathcal{F}$. 
\end{theorem}

For a linear concept class, the Rademacher complexity can be bounded as follows.

\begin{theorem}[\cite{KST:2008}] \label{rademachercomplexity}
	Let $\mathcal{X}$ be a subset of a Hilbert space equipped with inner product $\langle
	\cdot, \cdot \rangle$ such that for each $\textbf{x} \in \mathcal{X}$, $\langle \textbf{x}, \textbf{x}
	\rangle \leq X^2$, and let $\mathcal{W} = \{ \textbf{x} \mapsto \langle \textbf{x} , \textbf{w} \rangle
	~|~ \langle \textbf{w}, \textbf{w} \rangle \leq W^2 \}$ be a class of linear functions.
	Then it holds that
	%%
	\[
		\mathcal{R}_\textbf{m}(\mathcal{W}) \leq X \cdot W \cdot \sqrt{\frac{1}{m}}.
	\]
\end{theorem}

The following result is useful for bounding the Rademacher complexity of a smooth function of a concept class.

\begin{theorem}[\cite{BM:2002, LT:1991}]
\label{rademachercomplexity2}
	Let $\phi : \mathbb{R} \rightarrow \mathbb{R}$ be  $L_{\phi}$-Lipschitz
	and suppose that $\phi(0) = 0$. Let $\mathcal{Y} \subseteq \mathbb{R}$, and for a function $f \in \mathcal{Y}^{\mathcal{X}}$. 
	Finally, for $\mathcal{F} \subseteq \mathcal{Y}^{\mathcal{X}}$, let $\phi \circ \mathcal{F} = \{\phi \circ f \colon f \in \mathcal{F}\}$.
	It holds that $\mathcal{R}_\textbf{m}(\phi
	\circ \mathcal{F}) \leq 2 \cdot L_{\phi} \cdot \mathcal{R}_\textbf{m}(\mathcal{F})$.
\end{theorem}

\subsection{Kernel Methods}
We assume the reader has a basic working knowledge of kernel methods
(for a good resource on kernel methods in machine learning we refer the reader to
\cite{scholkopf2001learning}).  We denote a kernel function by $\mathcal{K}(\textbf{x},\textbf{x}') = \langle \psi(\textbf{x}), \psi(\textbf{x}') \rangle$ where $\psi$ is
the associated feature map and $\mathcal{H}$ is the
corresponding reproducing kernel Hilbert space (RKHS). 

Here we define two kernels and a few of their properties that we will use for our
analysis. First, we define a variant of the polynomial kernel, the
{\em multinomial kernel} due to Goel et al. \cite{goel2016reliably}:


\begin{definition}[Multinomial Kernel \cite{goel2016reliably}] \label{kernel1}
	Define $\psi_d \colon \mathbb{R}^n \to \mathbb{R}^{N_d}$, where $N_d = 1 + n + \cdots +
	n^d$, indexed by tuples $(k_1, \ldots, k_j) \in [n]^j$ for each $j \in \{0,
	1, \ldots, d \}$, where the entry of $\psi_d(\textbf{x})$ corresponding to tuple
	$(k_1, \ldots, k_j)$ equals $\textbf{x}_{k_1} \cdots \textbf{x}_{k_j}$.  (When $j = 0$ we have
	an empty tuple and the corresponding entry is $1$.) Define kernel ${\mathcal{MK}_d}$
	as follows:
	%
	\[
		{\mathcal{MK}_d}(\textbf{x}, \textbf{x}^\prime) = \langle \psi_d(\textbf{x}), \psi_d(\textbf{x}^\prime) \rangle = \sum_{j=0}^d (\textbf{x} \cdot \textbf{x}^\prime)^j.
	\]
Also define $\mathcal{H}_{{\mathcal{MK}_d}}$ to be the corresponding RKHS.
\end{definition}

It is easy to see that the multinomial kernel is efficiently computable. A multivariate polynomial $p$ of degree $d$ can be represented as an element $\textbf{v} \in \mathcal{H}_{{\mathcal{MK}_d}}$. Also, every $\textbf{v} \in \mathcal{H}_{{\mathcal{MK}_d}}$ can be interpreted as a multivariate polynomial of degree $d$ such that
\[
p(\textbf{x}) = \langle \textbf{v}, \psi_d(\textbf{x})\rangle = \sum_{\substack{(i_1, \dots, i_n) \in \{0, \ldots, d\}^n \\ i_i + \dots + i_n \leq d}} \beta(i_1, \dots, i_n) \textbf{x}_{1}^{i_1} \cdots \textbf{x}_n^{i_n}.
\]
where coefficient $\beta(i_1, \dots, i_n)$ is as follows,
\[
\beta(i_1, \dots, i_n) = \sum_{\substack{k_1, \ldots, k_j \in [n]^j
\\ j \in \{0, \ldots, d\}}}
\textbf{v}(k_1, \ldots, k_j).
\]
Here, $\textbf{v}(\cdot)$ is used to index the corresponding entry
in $\textbf{v}$. 
%Refer to \cite{goel2016reliably} for more details.

The following lemma is due to \cite{goel2016reliably}, following an
argument of Shalev-Shwartz et al. \cite{SSSS}: 

\begin{lemma}\label{lem:Bbound}
	%%
	Let $p(t) = \sum_{i=0}^d \beta_i t^i$ be a given univariate polynomial with
	$\sum_{i=1}^d \beta_i^2 \leq B^2$. For $\textbf{w}$ such that
        $||\textbf{w}|| \leq 1$, the polynomial $p(\textbf{w} \cdot
        \textbf{x})$ equals $\langle p_\textbf{w}, \psi(\textbf{x}) \rangle$ for some $p_\textbf{w} \in \mathcal{H}_{{MK_d}}$ with $|| p_{\textbf{w}} || \leq B$.
	%%
\end{lemma}
\noindent \textbf{Remark.} Observe that we can normalize the
  multinomial feature map such that $\forall \textbf{x} \in \mathcal{X}, \mathcal{MK}_d(\textbf{x},
  \textbf{x}) \leq 1$ for bounded space
  $\mathcal{X}$. More formally, $\max_{\textbf{x} \in \mathcal{X}}
  \mathcal{MK}_d(\textbf{x},\textbf{x}) = \max_{\textbf{x} \in \mathcal{X}} \sum_{j=0}^d
  ||\textbf{x}||^j \leq \sum_{j=0}^d
  X^j$ where $X =
  \max_{\textbf{x} \in \mathcal{X}} ||\textbf{x}||$, hence we can normalize using this value. Subsequently, in the above, $||p_{\textbf{w}}||$ will
  need to be multiplied by the same value. For
  $\mathcal{X} = \S^{n-1}$, the scaling factor is $d+1$
  \cite{goel2016reliably}.  Throughout the paper, we will assume the
  kernel to be normalized as discussed. \\

For our results on Multiple Instance Learning, we make use of the
following known kernel defined over sets of vectors:


\begin{definition}[Mean Map Kernel \cite{smola2007hilbert}]
Let $\mathcal{X}^*$ denote the Kleene closure of $\mathcal{X}$. 

The mean map kernel $\mathcal{K}_{\mathsf{mean}} \colon \mathcal{X}^* \times \mathcal{X}^* \rightarrow \mathbb{R}$ of kernel $\mathcal{K} \colon \mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}$ with feature vector $\psi \colon \mathcal{X} \rightarrow \mathcal{Z}$ is defined as,
\[
\mathcal{K}_{\mathsf{mean}}(S, T) = \frac{1}{|S||T|} \sum_{\textbf{s} \in S, \textbf{t} \in T} \mathcal{K}(\textbf{s},\textbf{t}).
\]
The feature map $\psi_{\mathsf{mean}} \colon \mathcal{X}^* \rightarrow \mathcal{Z}$ corresponding to this kernel is given by
\[
\psi_{\mathsf{mean}}(S) = \frac{1}{|S|} \sum_{\textbf{s} \in S} \psi(\textbf{s}).
\]
Also define $\mathcal{H}_{\mathsf{mean}}$ to be the corresponding RKHS.
\end{definition}
\noindent \textit{\textbf{Fact.} If $\forall \textbf{x}, \textbf{x}^\prime \in \mathcal{X}, \mathcal{K}(\textbf{x},\textbf{x}^\prime) \leq M$ then $\forall S, S^\prime \in \mathcal{X}^*, \mathcal{K}_{\mathsf{mean}}(S,S^\prime) \leq M$.}

\subsection{Approximation Theory}
We will make use of a variety of tools from approximation theory to
obtain specific embeddings of function classes into a RKHS.   The
following lemma for approximating the Boolean $\mathsf{sign}$ function
was given by \cite{daniely2015ptas}:

\begin{lemma}\label{lem:approxsign}
Let $a, \gamma, \tau > 0$. There exists a polynomial $p$ of degree $O\left( \frac{1}{\gamma} \cdot \log \left(\frac{1}{\tau}\right) \right)$ such that 
\begin{itemize}
\item For $x \in [−a, a]$, $|p({x})| < 1 + \tau$.
\item For ${x} \in [−a, a] \backslash [−\gamma \cdot a, \gamma \cdot a]$, $|p({x}) − \mathsf{sign}({x})| < \tau$.
\end{itemize}
\end{lemma}
The above lemma assumes $\mathsf{sign}$ takes on values $\{\pm 1 \}$,
but a simple linear transformation also works for $\{0,1\}$.

% A halfspace is a Boolean function $h: \mathbb{R}^n\rightarrow \{0, 1\}$ defined by a vector $\textbf{w}\in \mathbb{R}^n$ and threshold $\theta$, given input $\textbf{x} \in \mathbb{R}^n$, $h(\textbf{x}) = \mathsf{sign}(\textbf{w} \cdot \textbf{x} + \theta)$ where $\mathsf{sign}(a)$ is 0 if $a <0$ else 1. Given $\mathcal{X} \subseteq \mathbb{R}^n$ and halfspace $h$ over $\mathbb{R}^n$, $h$ is said to have margin $\rho$ with respect to $\mathcal{X}$ if $\rho = \min\{||z-y||: z \in \mathcal{X}, y \in \mathbb{R}^n, h(z) \neq h(y)\}/\max\{||z|| : z \in \mathcal{X}\}$. Let $h_{\textbf{w}_\textbf{i}}(\textbf{x})$ for $i \in [t]$ with $||\textbf{w}_\textbf{i}||_2 \leq 1$ be the $t$ halfspaces and $f_{\mathsf{AND}} = \mathsf{AND}(h_{\textbf{w}_\textbf{1}}, \ldots, h_{\textbf{w}_t}(\textbf{x}))$ equals the intersection. The following lemma due to Klivans and Servedio \cite{klivans2008learning} gives a construction of a polynomial whose sign always equals an
% intersection of halfspaces with a margin.  We give the proof as it is useful for a subsequent lemma.
% % \begin{lemma} \label{lem:inter}
% For $\rho >0$, there exists a polynomial $P_{\mathsf{AND}}$ of degree $O(\sqrt{1/\rho} \log t)$ such that, if each of the $t$ halfspaces has margin $\rho$ on $\mathcal{X} \subseteq \S^{n-1}$, then $\forall \textbf{x} \in \mathcal{X}$, $P_{\mathsf{AND}}(\textbf{x}) \geq 1/2$ if $f_{\mathsf{AND}}(\textbf{x}) = 1$ and  $P_{\mathsf{AND}}(\textbf{x}) \leq -1/2$ if $f_{\mathsf{AND}}(\textbf{x}) = 0$.  Constructively, $P_{\mathsf{AND}}$ is as follows, \[
% P_{\mathsf{AND}}(\textbf{x}) = t + \frac{1}{2} - \sum_{i=1}^t p(\textbf{w}_\textbf{i} \cdot \textbf{x})
% \]
% where $p(a) = T_r(1 - a)^{\lceil \log 2t \rceil}$ for $r = \lceil \sqrt{1/\rho} \rceil$ and $T_r$ is the $r$th Chebyshev polynomial of the first kind.
% \end{lemma}
% \begin{proof}
% We have $\forall i, \rho \leq |\textbf{w}_\textbf{i} \cdot \textbf{x}| \leq 1$. From the properties of Chebyshev polynomials, we know that $|T_r(1- a)| \leq 1$ for $a \in [0,1]$ and $T_r(1 - a) \geq 2$ for $ a \leq \rho$. Hence,
% \begin{itemize}
% \item If $f_{\mathsf{AND}}(\textbf{x}) = 1$, for each $i$, $\rho \leq \textbf{w}_\textbf{i} \cdot \textbf{x} \leq 1$ hence $|p(\textbf{w}_\textbf{i} \cdot \textbf{x})| \leq 1$, implying $P_{\mathsf{AND}}(\textbf{x}) \geq t + 1/2 - t = 1/2$.
% \item If $f_{\mathsf{AND}}(\textbf{x}) = 0$, then there exists $i$ such that $-1 \leq \textbf{w}_\textbf{i} \cdot \textbf{x} \leq \rho$, thus $p(\textbf{w}_\textbf{i} \cdot \textbf{x}) \geq 2^{\lceil \log 2t \rceil} \geq 2t$. Also observe that $\forall i, p(\textbf{w}_\textbf{i} \cdot \textbf{x}) \geq -1$. This implies $P_{\mathsf{AND}}(\textbf{x}) \leq t + 1/2 - 2t + t - 1 \leq -1/2$.
% \end{itemize}
% \end{proof}

% We extend the above lemma to give a threshold function for OR\footnote{A similar construction would hold for AND, with $P_{\mathsf{AND}}(S) = \frac{1}{2} + N - \frac{N}{|S|}\sum_{\textbf{s} \in S} p(\textbf{w} \cdot \textbf{s})$.} of a fixed halfspace with margin over a set of vectors. Let $h_\textbf{w}(\textbf{x}) = \mathsf{sign}(\textbf{w} \cdot \textbf{x})$ be a halfspace with $||\textbf{w}||_2 \leq 1$ and $f_{\mathsf{OR}}(S) = \mathsf{OR}(h_\textbf{w}(\textbf{s}_\textbf{1}), \ldots, h_\textbf{w}(\textbf{s}_t))$ represent the conjunction over any set $S = \{\textbf{s}_\textbf{1}, \ldots, \textbf{s}_t\}$ of vectors. Let $\mathcal{X} \subseteq \S^{n-1}$ over which the halfspace has margin.
% \begin{lemma} \label{lem:intermil}
% For $\rho, N >0$, there exists a function $P_{\mathsf{OR}}$ such that, if the halfspace $h$ has margin $\rho$ on $\mathcal{X} \subseteq \S^{n-1}$, then for all sets $S \subseteq \mathcal{X}^*$ such that $|S| \leq N$, $P_{\mathsf{OR}}(S) \geq 1/2$ if $f_{\mathsf{OR}}(S) = 1$ and  $P_{\mathsf{OR}}(S) \leq -1/2$ if $f_{\mathsf{OR}}(S) = 0$.  Constructively, $P_{\mathsf{OR}}$ is as follows, \[
% P_{\mathsf{OR}}(S) = -\frac{1}{2} - N + \frac{N}{|S|}\sum_{\textbf{s} \in S} p(\textbf{w} \cdot \textbf{s})
% \]
% where $p(a) = T_r(1 + a)^{\lceil \log 2N \rceil}$ for $r = \lceil \sqrt{1/\rho} \rceil$ and $T_r$ is the $r$th Chebyshev polynomial of the first kind.
% \end{lemma}
% \begin{proof}
% Similar to the previous proof, we have $\forall \textbf{x} \in \mathcal{X}, \rho \leq |\textbf{w} \cdot \textbf{x}| \leq 1$. From the properties of Chebyshev polynomials, we know that $|T_r(1+ a)| \leq 1$ for $a \in [-1,0]$ and $T_r(1 + a) \geq 2$ for $ a \geq \rho$. Hence,
% \begin{itemize}
% \item If $f_{\mathsf{OR}}(S) = 0$, for each $\textbf{s} \in S, -1 \leq \textbf{w} \cdot \textbf{s} \leq -\rho$ hence $|p(\textbf{w} \cdot \textbf{s})| \leq 1$, implying $P_{\mathsf{OR}}(S) \leq  -1/2  - N + N = -1/2$.
% \item If $f_{\mathsf{OR}}(S) = 1$, then there exists $\textbf{s} \in S$ such that $\rho \leq \textbf{w} \cdot \textbf{s} \leq 1$, thus $p(\textbf{w} \cdot \textbf{s}) \geq 2^{\lceil \log 2N \rceil} \geq 2N$. Also observe that $\forall \textbf{s} \in S, p(\textbf{w}\cdot \textbf{s}) \geq -1$. This implies $P_{\mathsf{OR}}(S) \geq  -1/2 - N + 2N - N + 1 \geq  1/2$ since $N \geq |S|$.
% \end{itemize}
% \end{proof} 

We state the following lemmas that bound the sum of squares of coefficients of a univariate polynomial:
\begin{lemma}[\cite{sherstov2012making}] \label{lem:dbound}
	Let $p(t) = \sum_{i=0}^d \beta_i t^i$ be a univariate polynomial of degree
	$d$. Let $M$ be such that $\displaystyle\max_{t \in [-1, 1]} |p(t)| \leq M$.
	Then $\displaystyle\sum_{i=0}^d \beta_i^2 \leq (d + 1) \cdot (4e)^{2d} \cdot
	M^2$. 
\end{lemma}


\begin{lemma} \label{lem:rbound}[Fact 3 \cite{klivans2008learning}]
	Let $p(t) = \sum_{i=0}^d \beta_i t^i$ be a univariate polynomial of degree
	$d$ such that $|\beta_i| \leq M$ for all $i \in [d]$. For any $r \in \mathbb{Z}^+$ consider $p^r(t) = \left(\sum_{i=0}^d \beta_i t^i\right)^r = \sum_{i=0}^{dr} \eta_i t^i$ then,
	 $\displaystyle\sum_{i=0}^{dr} \eta_i^2 \leq (Md)^{2r}$. 
\end{lemma}
\begin{proof}
We have $p^r(t) = \sum_{i_1, \cdots, i_r \in [d]} \beta_{i_1} \cdots \beta_{i_r} t^{i_1 + \cdots + i_r}$. It follows that $\left(\sum_{i=0}^d \beta_i t^i\right)^r = \sum_{i=0}^{dr} \eta_i t^i$ is bounded above by
\[
\left(\sum_{i_1, \cdots, i_r \in [d]} |\beta_{i_1} \cdots \beta_{i_r}|\right)^2 \leq M^{2r} \left(\sum_{i_1, \cdots, i_r \in [d]}1\right)^2 = (Md)^{2r}.
\]
\end{proof}
